Formalizing of Category Theory in Agda

The generality and pervasiness of category theory in modern mathematics makes it a frequent and useful target of formalization. It is however quite challenging to formalize, for a variety of reasons. Agda currently (i.e. in 2020) does not have a standard, working formalization of category theory. We document our work on solving this dilemma. The formalization revealed a number of potential design choices, and we present, motivate and explain the ones we picked. In particular, we find that alternative definitions or alternative proofs from those found in standard textbooks can be advantageous, as well as "fit" Agda's type theory more smoothly. Some definitions regarded as equivalent in standard textbooks turn out to make different "universe level" assumptions, with some being more polymorphic than others. We also pay close attention to engineering issues so that the library integrates well with Agda's own standard library, as well as being compatible with as many of supported type theories in Agda as possible.

==> makefile <==
.PHONY: all clean

TARGETS:=main.pdf template.pdf aim/main.pdf
TOREMOVE:=$(filter-out *.pdf,$(shell cat .gitignore))
TEXFILES:=$(subst ./,,$(shell find . -name '*.tex'))

all:main.pdf

${TARGETS}: %.pdf: %.tex $(filter-out $(subst .pdf,.tex,${TARGETS}),${TEXFILES})
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	bibtex $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

temp.pdf: temp.tex
	bibtex $(@:.pdf=) || true
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

FINDCMDPRE:=${foreach x, ${TOREMOVE}, -o -name '$x'}
FINDCMD:=${wordlist 2,${words ${FINDCMDPRE}},${FINDCMDPRE}}

clean:
	find . \( ${FINDCMD} \) -exec rm -rf {} +
	find . -name '_minted*' -exec rm -r {} +
	rm main.pdf

